A 3D Machine Learning based Volume Of Fluid scheme without explicit interface reconstruction

We present a machine-learning based Volume Of Fluid method to simulate multi-material flows on three-dimensional domains. One of the novelties of the method is that the flux fraction is computed by evaluating a previously trained neural network and without explicitly reconstructing any local interface approximating the exact one. The network is trained on a purely synthetic dataset generated by randomly sampling numerous local interfaces and which can be adapted to improve the scheme on less regular interfaces when needed. Several strategies to ensure the efficiency of the method and the satisfaction of physical constraints and properties are suggested and formalized. Numerical results on the advection equation are provided to show the performance of the method. We observe numerical convergence as the size of the mesh tends to zero $h=1/N_h\searrow 0$, with a better rate than two reference schemes.

==> style.tex <==
\ProvidesPackage{style}

\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage[latin1]{inputenc}
\usepackage[english]{babel}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{floatflt,epsfig}
\usepackage{verbatim}
\usepackage{dsfont}
\usepackage{subcaption}
\usepackage{xcolor}   % for \textcolor
\usepackage[labelformat=parens,labelsep=quad,skip=3pt]{caption}
\usepackage{listings}
\usepackage[inner=25mm,
	outer=25mm]{geometry}
%\usepackage{empheq}
\usepackage{soul}
\usepackage{bbm}
%\usepackage{natbib}
%\usepackage{subfig}

%\usepackage[hidelinks]{hyperref} 
\usepackage{mathtools}
\usepackage[shortlabels]{enumitem}
%\usepackage{float}

\usepackage[figurename=Fig.,labelfont=bf]{caption}

%\usepackage{hyperref}       % hyperlinks
%\hypersetup{
%    colorlinks,
%    linkcolor={red!50!black},
%    citecolor={blue!50!black},
%    urlcolor={blue!80!black}
%}
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{bbm}
\lstset{
  basicstyle=\ttfamily,
  columns=fullflexible,
 % frame=single,
  breaklines=true,
  postbreak=\mbox{\hspace{2cm}\textcolor{red}{$\hookrightarrow$}\space},
}


%%Header styles
%\usepackage{fancyhdr}
%\setlength{\headheight}{15pt}
%\pagestyle{fancy}
%%\renewcommand{\chaptermark}[1]{\markboth{#1}{}}
%%\renewcommand{\sectionmark}[1]{\markright{#1}{}}
%\fancyhf{}
%\fancyhead[LE,RO]{\thepage}
%\fancyhead[RE]{\textbf{\textit{\nouppercase{\leftmark}}}}
%%\fancyhead[LO]{\textbf{\textit{\nouppercase{\rightmark}}}}
%\fancypagestyle{plain}{ %
%\fancyhf{} % remove everything
%\renewcommand{\headrulewidth}{0pt} % remove lines as well
%\renewcommand{\footrulewidth}{0pt}}

%makes available the commands \proof, \qedsymbol and \theoremstyle
%\usepackage{amsthm}

%Ruler
\newcommand{\HRule}{\rule{\linewidth}{0.5mm}}

%\newtheoremstyle{break}
%  {\topsep}{\topsep}%
%  {\itshape}{}%
%  {\bfseries}{}%
%  {\newline}{}%
%\theoremstyle{break}

%Lemma definition and lemma counter
\newtheorem{lemma}{Lemma}[section]

%Definition counter
\theoremstyle{definition}
\newtheorem{definition}[lemma]{Definition}

%Corolary counter
\newtheorem{corollary}[lemma]{Corollary}

%Theorem counter
\newtheorem{theorem}[lemma]{Theorem}

%Proposition counter
\newtheorem{proposition}[lemma]{Proposition}

%Property counter
\newtheorem{property}[lemma]{Property}

%Assumption counter
\newtheorem{assumption}[lemma]{Assumption}

%Remark counter
\newtheorem{remark}[lemma]{Remark}

%Commands for naturals, integers, topology, hull, Ball, Disc, Dimension, boundary and a few more
\newcommand{\E}{{\mathcal{E}}}
\newcommand{\F}{{\mathcal{F}}}
\newcommand{\M}{{\mathcal{M}}}
\newcommand{\T}{{\mathcal{T}}}
\newcommand{\MM}{\mathcal{M}}
\newcommand{\Bs}{{\mathcal{B}}}
\newcommand{\R}{{\mathbb{R}}}
\newcommand{\Q}{{\mathbb{Q}}}
\newcommand{\Z}{{\mathbb{Z}}}
\newcommand{\Nt}{{\mathbb{N}}}
\newcommand{\B}{{\mathbf{B}}}
\renewcommand{\S}{{\mathbf{S}}}
\newcommand{\K}{{\mathfrak{C}}}
\newcommand{\N}{{\mathbb{N}}}
\newcommand{\I}{{\mathbf{I}}}
\renewcommand{\L}{{\mathcal{L}}}
\renewcommand{\P}{{\mathbb{P}}}
\newcommand{\C}{{\mathbb{C}}}

\newcommand{\uu}{{\mathbf u}}
\newcommand{\vv}{{\mathbf v}}
\newcommand{\ww}{{\mathbf w}}
\newcommand{\xx}{{\mathbf x}}
\newcommand{\mypm}{\mathbin{\ooalign{\lower.58ex\hbox{$-$}\cr\raise.3ex\hbox{$+$}\cr}}}
\DeclareMathOperator*{\avg}{avg}
\DeclareMathOperator*{\abs}{abs}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argsup}{arg\,sup}
\DeclareMathOperator*{\arginf}{arg\,inf}
\DeclareMathOperator*{\esssup}{esssup}
\newcommand\restrict[1]{\raisebox{-.5ex}{$|$}_{#1}}

%Example cenvironment
%\theoremstyle{remark}
%\newtheorem{style}{style}

%Example counter
\newcommand{\reiniciar}{\setcounter{example}{0}}

\setcounter{tocdepth}{4}
\setcounter{secnumdepth}{4}

\usepackage[labelformat=simple]{caption}
\renewcommand{\thefigure}{\arabic{figure}}
\renewcommand{\thesubfigure}{\thefigure.\alph{subfigure}}

\newcommand{\footremember}[2]{%
    \footnote{#2}
    \newcounter{#1}
    \setcounter{#1}{\value{footnote}}%
}
\newcommand{\footrecall}[1]{%
    \footnotemark[\value{#1}]%
} 

\newcommand{\NN}{{\mathcal{N\hspace{-0.065cm}N}\hspace{-0.055cm}}}
\newcommand{\x}{{\mathbf{x}}}

\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}



